Evaluating kernels on Xeon Phi to accelerate Gysela application

This work describes the challenges presented by porting parts ofthe Gysela code to the Intel Xeon Phi coprocessor, as well as techniques used for optimization, vectorization and tuning that can be applied to other applications. We evaluate the performance of somegeneric micro-benchmark on Phi versus Intel Sandy Bridge. Several interpolation kernels useful for the Gysela application are analyzed and the performance are shown. Some memory-bound and compute-bound kernels are accelerated by a factor 2 on the Phi device compared to Sandy architecture. Nevertheless, it is hard, if not impossible, to reach a large fraction of the peek performance on the Phi device,especially for real-life applications as Gysela. A collateral benefit of this optimization and tuning work is that the execution time of Gysela (using 4D advections) has decreased on a standard architecture such as Intel Sandy Bridge.

==> gysela_equations.tex <==
\subsection{Parallel solving of Vlasov equation}

Our gyrokinetic model considers as main unknown a distribution
function $\fbar$ that represents the density of ions at a given phase
space position.  This function depends on time and on $5$ other
dimensions.  First, 3 dimensions in space, $r$ and $\theta$ are the
polar coordinates in the shortest cross-section of the torus (called
poloidal section), while $\varphi$ refers to the angle in the largest
cross-section of the torus. Second, velocity space has two dimensions:
$v_{\parallel}$ being the velocity along the magnetic field lines (one
has $\textstyle{v_{\parallel}=\textrm{d}\varphi/\textrm{d}t}$), and
$\mu$ the magnetic moment corresponding to the action variable
associated with the gyrophase.  The time evolution of the
guiding-center 5D gyroaveraged distribution function
$\fbar_t(r,\theta,\varphi,v_{\parallel},\mu)$ is governed by the
so-called gyrokinetic equation\,\cite{hahm,virginie}~:

\vspace*{-0.1cm}
\begin{equation}
  \D{\fbar}{t} + \K{r}{t}\D{\fbar}{r} + \K{\theta}{t}\D{\fbar}{\theta}+
  \K{\varphi}{t}\D{\fbar}{\varphi} + \K{v_{\parallel}}{t}\D{\fbar}{v_{\parallel}} =
  0. 
\label{vlasoveq}
\end{equation}

\vspace*{-0.1cm} In this Vlasov gyrokinetic equation, $\mu$ acts as a
parameter because it is an adiabatic motion invariant.  Let us denote
by $N_\mu$ the number of $\mu$ values, we have $N_\mu$ independent
Eq. \ref{vlasoveq} to solve at each time step. The function
$\fbar$ is periodic along $\theta$ and $\varphi$. Vanishing
perturbations are imposed at the boundaries in the non-periodic
directions $r$ and $v_\parallel$.


GYSELA is a global nonlinear electrostatic code which solves the
gyrokinetic equations with a semi-Lagrangian
method\,\mbox{\cite{vlasovia06,virginie}}. We combine this
with a second order in time Strang splitting method. The
solving of the Vlasov Eq.~(\ref{vlasoveq}) is not the topic of this
paper and we refer the reader to \cite{guillaume,virginie} for
detailed descriptions. We will only recall a few issues concerning the
parallel domain decomposition used by this Vlasov solver.  Large data
structures are used in GYSELA, the main ones are: the 5D data $\fbar$,
and the 3D data as the electric potential $\Phi$. 
Let $\NA_r$, $\NA_\theta$, $\NA_\varphi$,
$\NA_{v_{\parallel}}$ be respectively the number of points in each
dimension $r$, $\theta$, $\varphi$, ${v_{\parallel}}$. 

In the Vlasov solver, we give the
responsibility of each value of $\mu$ to a given set of MPI
processes\,\cite{guillaume} (a MPI communicator). We fixed that there
are always $\Nmu$ sets, such as only one $\mu$ value is
attributed to each communicator. Within each set, a 2D domain
decomposition allows us to attribute to each MPI Process a subdomain
in $(r,\theta)$ dimensions. Thus, a MPI process is then responsible
for the storage of the subdomain defined by
{\footnotesize $\fbar(r=[i_{start},i_{end}],\theta=[j_{start},j_{end}],\varphi=*,v_\parallel=*,\mu=\mu_{value})$}.
The parallel decomposition is initially set
up knowing local values $i_{start}, i_{end},
j_{start}, j_{end},\mu_{value}$. They are derived from a classical
block decomposition of the $r$ domain into $\Npr$
pieces, and of the $\theta$ domain into $\Npt$
subdomains. The numbers of MPI processes used during one run is equal to
$\Npr{}\times{}\Npt\times{}\Nmu{}$. The OpenMP
paradigm is used in addition to MPI (\NT{}~threads in each MPI process) 
to bring fine-grained parallelism in addition. 


\subsection{Quasineutrality equation}

The quasineutrality equation and parallel Ampere's law close the
self-consistent gyrokinetic Vlasov-Maxwell system. However, in an
electrostatic code, the Maxwell field solver reduces to the numerical solving
of a Poisson-like equation (theoretical foundations are presented
in\,\cite{hahm}).  In tokamak configurations, the plasma
quasineutrality (denoted QN) approximation is currently assumed
\cite{virginie,hahm}.  Electron inertia is ignored, which means that
an adiabatic response of electrons is supposed. We define the operator
$\textstyle{\nabla\!}_{\perp}=(\pa_r,\frac{1}{r}\pa_{\theta})$. We
note $n_0(r)$ the equilibrium density, $B_0$ the magnetic field at the
magnetic axis and $T_e(r)$ the electronic temperature. We have also
$B(r,\theta)$ the magnetic field, $J_0$ the Bessel function of first
order and $k_{\perp}$ the transverse component of the wave vector.
Hence, the QN equation can be written in dimensionless variables 
\be
-\frac{1}{n_0(r)}\nabla_{\perp}\,.\left[\frac{n_0(r)}{B_0}\nabla_{\perp}\Phi(\rad,\theta,\varphi)\right]+\frac{1}{T_e(r)}\left[\Phi(r,\theta,\varphi)-\left<\Phi\right>_{\theta,\varphi}(r)\right]
= \brho(r,\theta,\varphi)
\label{qneq}
\ee
where $\brho$ is defined by 
\be
\label{brho}
\brho(r,\theta,\varphi)=\frac{2\pi}{n_0(r)}\int B(r,\theta)d\mu\int
dv_{\parallel}
J_0(k_{\perp}\sqrt{2\mu})(\bar{f}-\bar{f}_{eq})(r,\theta,\varphi,v_{\parallel},\mu).
\ee with $\bar{f}_{eq}$ representing local ion Maxwellian equilibrium,
and $\left<\right>_{\theta,\varphi}$ the average onto the variables
$\theta,\varphi$.  The presence of the non-local term $\left<\Phi\right>_{\theta,\varphi}(r)$ couples
$(\theta,\varphi)$ dimensions and penalizes the parallelization. We employ a
solution based on FFT to overcome this
problem. But this method is valid only in polar coordinates and not adapted to all
geometries\,\cite{lin}. The QN solver includes two parts. First, the
function $\brho$ is derived taking as input function $\bar{f}$ that comes
from the Vlasov solver. In Eq.~(\ref{brho}) specific methods
(\textit{e.g.} see\,\cite{RR-7591}) are used to evaluate the
gyroaverage operator $J_0$ on $(\bar{f}-\bar{f_{eq}})$.  Second, the
3D electric potential $\Phi$ is derived. We use the parallel algorithm
introduced in \cite{latu11a}.

In the following, we will refer to several  data as \tit{3D
  field data}. They are produced and distributed over the parallel
machine just after the QN solver. These field data sets, 
namely: {\footnotesize
  $\Phi, \D{J_0(k_{\perp}\sqrt{2\mu})\Phi}{r},
  \D{J_0(k_{\perp}\sqrt{2\mu})\Phi}{\theta},
  \D{J_0(k_{\perp}\sqrt{2\mu})\Phi}{\varphi}\ ,$} are distributed on
processes in a way that exclusively depends on the parallel domain
decomposition chosen in the Vlasov solver. Indeed, they are inputs for
the Vlasov Eq. (\ref{vlasoveq}), and they play a major
role in terms  {\footnotesize $\K{r}{t}, \K{\theta}{t}, \K{\varphi}{t},
\K{v_{\parallel}}{t}$} not detailed here. So we fix that the subdomain
owned by each MPI process has the form  
{\footnotesize  $(r=[i_{start},i_{end}],
\theta=[j_{start},j_{end}], \varphi=*)$} for the 3D field data.

\subsection{\label{gys_eq:parts}Main parts of the code}


The application can be seen as a collection of physical features and
solvers that model and mimic a set of physics phenomena taking place inside a
Tokamak plasma. Here is a list of the major components of the \gy code~:
\begin{itemize}
\item \textbf{Vlasov solver} -  Vlasov equation is a transport equation
  posed in the the phase space (see Eq. \ref{vlasoveq}). The Vlasov solver uses a semi-Lagrangian approach and a splitting of Strang as main ingredients. It is mixed with some of the components that follows, such that it can also be called a \tit{Boltzmann solver}. Its role is to move the distribution function $\bar{f}$ one time step forward.
\item \textbf{Field solver} -  The QN solver is based on a Poisson solver. It gives the electric potential $\Phi$ generated by the distribution of particles at a time step taking as input the distribution function $\bar{f}$.
\item \textbf{Derivatives computation} -  The derivatives of gyroaveraged electric potential (generated by the Field solver) are used to establish the particle trajectories inside the Vlasov solver. The derivatives of $J_0(k_{\perp}\sqrt{2\mu})\Phi$ are computed along the $r$, $\theta$ and $\varphi$ directions.
\item \textbf{Sources} -  Source terms are used to model the external heating of the Plasma. Theses terms are injected as a right hand side of the Eq. \ref{vlasoveq}.
\item \textbf{Collisions} -  Core plasmas are widely believed to be collisionless, but recent evidence from experimental side and from modelisation are contributing to alter this idea. Ion-ion collisions are included through a reduced Fokker-Planck collision operator. The collisions are added to the right hand side of the Eq. \ref{vlasoveq}.
\item \textbf{Diffusions} - In order to model radial boundary conditions, diffusion operators are used on buffer regions to relax quickly towards a thermal bath. Buffer regions represent a small radial fraction of the minor radius.
\item \textbf{Diagnostics} - Physically relevant quantities are computed at a given time frequency in the code. This part, named \tit{Diagnostics}, derives and ouputs some files taking as input distribution function and electric potential.
%These modifications allow exploring more realistic tokamak turbulence regimes.
\end{itemize}

The Vlasov solver is one of the first computation intensive part of the code. For large physical cases, for which the parallel scalability is fine, the Vlasov solver represents more than 50\% of the computational cost even with thousands of nodes. The load balancing is quite good up to 65k cores using an hybrid OpenMP/MPI approach in each of the component of \gy{}. The largest parallel overheads originate from communication issues and synchronization of all nodes in some subroutines. The communications required are mainly due to the change of domain decompositions we are dealing with in the \gy{} code (mainly between field solver and Vlasov solver as we shall see).


%%% Local Variables:
%%% TeX-master: "mic-esaim"
%%% End:

